Photonics-integrated terahertz transmission lines

Modern communication and sensing technologies rely on connecting the optical domain with the microwave domain. Terahertz technologies, spanning increased frequencies from 100 GHz to 10 THz, are critical for providing larger bandwidths and faster switching capabilities. Despite progress in high-frequency electronic sources and detectors, these technologies lack a direct link to the optical domain, and face challenges with increasing frequencies (> 1 THz). Nonlinear processes, such as optical rectification, offer potential solutions for terahertz generation but are currently limited to discrete components based on bulk nonlinear crystals, missing out miniaturisation opportunities from integration of optical circuits with terahertz ones. We address this challenge by integrating phase-matched terahertz transmission lines with photonic circuits in a single hybrid architecture on the thin-film lithium niobate~(TFLN) platform. This design demonstrates phase-matched, broadband terahertz emission spanning four octaves (200 GHz to 3.5 THz) through broadband down-conversion of optical signals at telecommunication wavelengths. The micron-sized transmission lines provide terahertz field confinement with minimal radiative loss, enabling compact THz cavities embedded in integrated photonic circuits. This integration is crucial for leveraging photonics' advantages in low-noise, low-loss, and high-speed operations for terahertz generation. Our platform can readily be integrated with other mature photonics components, such as electro-optic modulators, frequency comb sources, or femtosecond sources to pave the way for compact, power-efficient, and frequency-agile broadband sources with applications in telecommunications, spectroscopy, quantum electrodynamics and optical computing.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
